Environmental drivers of systematicity and generalization in a situated agent

The question of whether deep neural networks are good at generalising beyond their immediate training experience is of critical importance for learning-based approaches to AI. Here, we consider tests of out-of-sample generalisation that require an agent to respond to never-seen-before instructions by manipulating and positioning objects in a 3D Unity simulated room. We first describe a comparatively generic agent architecture that exhibits strong performance on these tests. We then identify three aspects of the training regime and environment that make a significant difference to its performance: (a) the number of object/word experiences in the training set; (b) the visual invariances afforded by the agent's perspective, or frame of reference; and (c) the variety of visual input inherent in the perceptual aspect of the agent's perception. Our findings indicate that the degree of generalisation that networks exhibit can depend critically on particulars of the environment in which a given task is instantiated. They further suggest that the propensity for neural networks to generalise in systematic ways may increase if, like human children, those networks have access to many frames of richly varying, multi-modal observations as they learn.

==> scratch.tex <==
\section{Examples of systematic generalisation}
test

% \paragraph{A generalisable notion of lifting} A key aspect of language understanding is the ability to flexibly combine predicates with arguments; verb-noun binding is perhaps the canonical example. Verbs typically refer to processes and actions, so to study this phenomenon in learning agents we move to simulated 3D room built in the Unity game engine [REF]. In this environment, the agent observes the world from a first-person perspective, the objects are 3D renderings of everyday things, the environment has simulated physics enabling objects to be picked-up, moved and stacked, and the agent's action-space consists of 15 relatively fine-grained actions such as XXXX \footnote{See appendix for a full list of the action space}. In this room, executing a simple instruction like \texttt{find a toothbrush}, which could be accomplished in 6 actions in the grid world, would require approximately 35 small movements in the Unity room. 

% 'Lifting' is a simple verb-like motor process that is easily studied in this room. We consider the instruction `lift a helicopter' to be successfully executed if the agent gets close enough to the helicopter to pick it up, raises it above a minimum height of 0.5m and holds it there for 2 seconds (requiring multiple find-grained actions once the helicopter is located). Similarly, the instruction `find a helicopter' is realised if the agent moves within two metres of a helicopter and fixes its gaze (as determined by a ray cast from the agent's visual field) while remaining withing the 2m proximity for (15 timesteps) \emph{without lifting the object during this time}. To measure how general the acquired notion of `lifting' is, we train the agent to `find' each of a set $X = X_1 \cup X_2 $ of different objects (allowing the agent to learn to ground objects to their names) and to `lift' a subset $X_1$ of those objects in trials in a small room containing two objects positioned at random (one `correct' according to the instruction, and one `incorrect'). A positive reward is emitted from the environment if the agent carries out the correct process (find/lift) on the correct, and the episode ends (with no reward) if the agent carries out that process on the incorrect object. We then evaluate its ability to extend its notion of lifting (zero-shot) to objects $x \in X_2$. In a variant of this experiment, we train the agent to lift all of the objects in $X$, but when referred to by their color (`lift a green object`), and to find all of the objects in $X$ according to either shape or color (`find a pencil`, `find a blue object`). We again test on whether the agent can lift objects $x \in X_2$ according to their shape (so the test trials in both variants are the same). As shown Fig~\ref{fig:put_lift_generalisation}, in both variants the agent generalises with near-perfect accuracy. Thus the agent has acquired a notion of what it is to lift an object (and how this binds to the word `lift`) with sufficient generality that it can apply it to novel objects, or to familiar objects with novel modes of linguistic reference, without further training.


% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/put_lift_generalisation.png}
%     \caption{How test performance corresponds to training performance as an agent learns to zero-shot predicate-argument binding for (a) `lifting' in two variants: (1) training instructions are like `find a spaceship, find/lift a pencil', testing instructions are like `lift a spaceship'. (2) training instructions are like `find a spaceship/lift a green object', testing instructions are like `lift a spaceship'. (b) `putting': training instructions are like `put a spaceship on the bed', `lift a pencil', testing instructions are like `put a pencil on the bed'.}
%     \label{fig:put_lift_generalisation}
% \end{figure*}


% \paragraph{A generalisable notion of putting}
% \label{sec:put_lift_generalisation}
% We explored the limits of this sort of predicate-object binding by placing two large, flat objects (a bed and a tray) in the room and training an agent place one of three smaller objects on top of those objects (all objects are placed initially at random). As before, a positive reward is emitted by the environment if the agent places the correct small object on the bed or the tray according to the instruction. If an incorrect object is placed on the bed or tray, the episode ended with no reward. To test generalisation in this case, we trained the agent to lift each of a set $X = X_1 \cup X_2$ of smaller objects (as in the previous experiment) and then to put some subset $X_1 \cup X$ of those objects on both the bed and the tray as instructed. We then measured its performance (with no learning) in trials where it was instructed to put objects from $X_2$ onto either the bed or the tray. Surprisingly, we found that the agent was able to place objects with over 90\% accuracy onto the bed or the tray zero-shot as instructed (Fig~\ref{fig:put_lift_generalisation} (b)). This generalisation requires the agent to bind its knowledge of objects (referred to by nouns, and acquired in the lifting trials) to a complex control process (acquired in the training putting trials) -- involving locating the correct target receptacle. moving the object above it (avoiding obstacles like the bed-head) and dropping it gently. An important caveat here is that control in this environment, while fine-grained, is far simple than the real world; in particular the process required to lift an object does not depend on the shape of that object (only its extent, to a degree). Once the objects are held by the agent, however, their shape becomes somewhat more important and placing something on top of something else, avoiding possible obstacles that could knock the object from the agent's grasp, is a somewhat object-dependent process. The video [XXX] gives a better sense of thee complexity of this process.


% \paragraph{A general notion of negation}
% Negation is an important aspect of language understanding. Rummelhart showed that a two-layer feedforward network (with sufficient hidden units) can learn to predict the negation of binary patterns. We translate Rummelhart's experiment to the context of an embodied agent with continuous (visual) input and, importantly consider not only the ability to learn to negate, but also to \emph{generalise} this notion to unseen arguments. To do so, we generated trials in the Unity room with two different objects positioned at random and instructions of the form \texttt{find a helicopter} (in which case  the agent was rewarded for locating and fixing gaze on the helicopter) and \texttt{find} [something that is] \texttt{not a helicopter} (in which case there was a helicopter in the room but the agent was rewarded for locating the other object). 

% Like Rummelhart, we found that it was unproblematic to train an agent to respond correctly to both positive (\texttt{find a helicopter}) and corresponding negated instructions \texttt{find not a helicopter}. We also explored generalisation of the netation principle, by training the agent to follow instructions \texttt{find a x} for all $x \in X$ and and negated instructions \texttt{find a not x} for only $x \in X_1$ (where $X = X_1 \cup X_2$, and $X_1, X_2 \cap = \emptyset$), the testing how it interpreted negative commands for $x \in X_2$. 

% \begin{wraptable}{r}{7cm}
% \begin{tabular}{ccc}\\\toprule
% Training set & Train accuracy & Test accuracy \\\midrule
% 6 words & 1.00 & 0.40\\  \midrule
% 40 words & 0.97 & 0.60\ \  \midrule
% 100 words & 0.91 & 0.78 \\  \bottomrule
% \end{tabular}
% \caption{A wrapped table going nicely inside the text.}\label{tab:negation}
% \end{wraptable} 


% We found that the emergence of (a systematic notion of) negation was less immediate than the predicates involved in previous experiments. Specifically, when $X_1$ contained only a few objects ($\|X_1\| = 5$), the agent interpreted negated instructions involving objects from $X_2$ (where $\vert X_2\vert == 6$)  with \emph{below chance} accuracy: i.e, for objects $x_2 \in X_2$, in response to the instruction \texttt{find a not $x_2$} the agent was more likely to find the object $x_2$ than the other object in the room. We suspect in such cases that the agent simply infers that \textt{not x} refers to the set $\{y \in X_1 : x \neq y\}$ (this highly non-compositional interpretation would leave it hopeless when interpreting instructions involving the members of $X_2$). Importantly, however, for ($\|X_1\| = 40$) the agent achieved above chance interpretation of held-out negated instructions. We then increased the agent's experience by including an additional 60 visual assets from the \textit{ShapeNet} dataset in the training regime. This increased accuracy on the same set of held-out negated instructions to $0.78$ (Fig~\ref{tab:negation}). While this performance may seem notably less than perfect, it is worth noting that humans perform with approximately 80\% accuracy on a range of systematicity tests relating to language [REF - Lake et al]. 


% \section{Principles underlining generalisation}
% The experiments thus far confirm the possibility of systematic generalisation in embodied agents. However, it is also important to understand the aspects of our experiments that contribute to the emergence of this systematicity so that future work can better rely on such behaviour, particularly since it is not \emph{always} observed when training neural networks. To this end, we conducted additional experiments across three different environments, which allowed us to identify four factors that contribute to the systematicity of an agent: \emph{abstraction across the training set}, \emph{environmental realism}, \emph{the agent perspective} and \emph{multimodality}.

% \subsection{Abstracting across the training set}

% In all of our experiments, our agents are trained with a degree of procedural variation in the tasks that they attempt and certain environmental factors. To show how this variation can drive systematicity even in highly controlled domains, we designed a simple grid-world experiment that tested our agent's ability to combine shape and color words in a systematic way\footnote{This ability of multi-modal agents to generlize shape-color composition has already been established in several prior studies [REF]}. In our grid world, the agent receives a RGB pixel representation of the world from a top-down perspective, including a square indicating its current position. The agent can take one of four actions (\texttt{UP, DOWN, LEFT, RIGHT}) to move around the world. At the start of each episode, the agent receives a two-symbol instruction (\texttt{red triangle}) indicating the colour and the shape of the target object. If the agent moves into the target object before the episode ends, it receives a positive reward, and if it moves into the (incorrect) distractor object or the time runs out it receives no reward. Each episode ends after 30 timesteps or when the agent moves into the square occupied by one of the objects. Over the course of multiple episodes, the agent learns how these symbols correspond to its visual observations and develop a language-conditional policy of moving towards the correct object when instructed. 

% To evaluate generalisation, the available colors and shapes in the environment were partitioned into sets $S = \mathbf{s} \cup \hat{\mathbf{s}}$ and $C = \mathbf{c} \cup \hat{\mathbf{c}}$. We then train the agent on episodes with instructions sampled from one of the sets $ \mathbf{c} \times \mathbf{s}$, $\hat{\mathbf{c}} \times \mathbf{s}$ or $ \mathbf{c} \times \hat{\mathbf{s}}$, and, once trained, we evaluate its performance on instructions from $ \hat{\mathbf{c}} \times \hat{\mathbf{s}}$. Importantly, to ensure all parts of the referring expression in the instruction are necessary, during both training and testing the agent faces trials in which the distractor object either matches the color of the target object or the shape of the target object. Figure X shows that the agent exhibits good ability to generalise (recombining shape and color terms into novel combinations) even when the sets $\mathbf{s}, \mathbf{c}, \hat{\mathbf{s}}, \hat{\mathbf{c}}$ contain a small number of factors from which to learn. 

% \begin{table}
% 	\begin{minipage}{0.25\linewidth}
% 		\centering
% 		\includegraphics[width=40mm]{figures/color_shape.png}
% 		%\captionof{figure}{2-D scatterplot of the Student Database}
% 		\label{ }
% 	\end{minipage}\hspace*{\fill}
% 	\begin{minipage}{0.2\linewidth}
% 		\label{table:student}
% 		\centering
% 	    \footnotesize{
% 		\begin{tabular}{llllrr}
% 			\toprule
% 			C  & S & \hat{C} & \hat{S} & Tr & Te \\
% 			&&&&&\midrule\\
% 			&&&&&\bottomrule
% 		}
% 		\end{tabular}
% 	\end{minipage}\hspace*{\fill}
% 	\begin{minipage}{0.25\linewidth}
% 		\centering
% 		\includegraphics[width=40mm]{color_shape_sunflower.png}
% 		%\captionof{figure}{2-D scatterplot of the Student Database}
% 		\label{ }
% 	\end{minipage}\hspace*{\fill}
% 	\begin{minipage}{0.2\linewidth}
% 		%\caption{Student Database}
% 		\label{table:student}
% 		\centering
% 	    \footnotesize{
% 		\begin{tabular}{llrr}
% 			\toprule
% 			C  & S & Tr & Te \\
% 			\midrule
% 			 2 & 2  & 1.00 & 0.64  \\
% 			 9  & 2  & 1.00 & 0.80 \\
% 			\bottomrule
% 		}
% 		\end{tabular}
% 	\end{minipage}
% \caption{Zero-shot generalisation of (color-shape) object referring expressions for different training regimes. Left almost perfect systematic generalisation is observed when all shapes are observed during training with some variety of different colors. Right, generalisation is above 80\% accuracy (chance = 0.5) for shapes observed with a single colour during training; this capacity grows with the number of colors ($\vert \mathbf{c} \vert$) that \emph{other} shapes in the training set are observed with. All scores reflect the mean performance of the top three of five agent replicas (ranked by performance on the training set) per condition.}
% \end{table}

% The assumption that all objects and shape-words can be encountered in a range of different colours is not particularly realistic. In the experience of a human learner, certain objects might be experienced in multiple colours (such as toys) while others (such as fruits) will have a single colour, but we can understand expressions like \emph{purple banana} without direct experience of such a thing. To test this capacity, we trained the agent on instructions sampled either from a set $ \mathbf{c} \times \mathbf{s}$ or from a set $ \{c\} \times \hat{\mathbf{s}}$ where $c$ is a single color. We then evaluated the trained agent on episodes with target object descriptions from $\mathbf{c}\times \hat{\mathbf{s}}$. The shapes in the set $\hat{\mathbf{s}}$ play the role of banana in the example above, while $c$ is its typical color yellow. As shown in Fig~\ref{fig:blue_sunflower}, we find that the agent can understand the `banana` terms $\hat{\mathbf{s}}$ described in conjunction with colors other than yellow in 80\% of episodes. Interestingly, this capacity increases as the variety of colors that \emph{other} shapes in the training set are observed with increases. This suggests that the experience of shapes that vary widely in color (the fully green area of the training regime in Fig~\ref{fig:blue_sunflower}) are critical to the development of color as a separable and recombinable aspect of experience, the knowledge of how color words refer to this, and the ability to apply this knowledge, in theory, to any shape whatsoever. 


% \subsection{Environmental realism}
% The `blue sunflower` analysis shows that agents operating in a grid-world can learn to generalize systematically given sufficient variation in theiry training data. However, in the cases the more realistic environment 3D Unity room, we observed systematic generalisation with making a particular effort to involve many factors of variation in the training data. This suggests that environmental realism in general (rather than explicit variation in directly-relevant factors or words) might play an important role in stimulating emergent systematicity.

% To test this hypothesis explicitly, we compared the generalisation of an agent trained to lift objects and to put them on a bed (as in Section~\ref{sec:put_lift_generalisation}), when trained in both a  (more realistic) Unity room and a (more abstract) grid world. At a certain level of abstraction, the tasks in the two environments were identical; each episode involved three red objects and a white object positioned at random in a room. In `lifting' trials, the agent in both cases had to visit a specific red object, and in `putting' trials, the agent had to pick up a specific object and move with that object to the bed. There was a total of seven possible red objects in both cases, of which all were involved with `lifting' trials during training but only three in `putting' trials. The test trials consisted of `putting' trials with the remaining four objects. While the task are identical at a conceptual (and linguistic) level, the experience of an agent doing the task in the the grid world was quite different from that in the Unity room. In the grid world, the agent observed the whole world (including itself) from above, and could move to only 49 possible locations by taking one of four possible actions. 

% As shown in figure X, agents in both conditions were able to master the training set with almost perfect performance. However, on the test set, the performance of the agent in the Unity room was far better than the agent in the grid world. Failure cases of agent in the grid world can be observed in the video REF; it typically exhibits less certainty, putting the wrong object on the bed or running out of time before it is able to make a decision. 

% Many studies that have observed limited systematic generalisation in neural network-based models involve synthetic symbolic data [REF] or abstract grid environments [REF]. This led to a hypothesis that emergent systematicity might in fact be supported by environmental richness. 

% \begin{minipage}[ht!]{\textwidth}
% \begin{minipage}[b]{0.6\textwidth}
% \centering
%     \includegraphics[width=8cm]{figuures/grid_vs_unity.png}
% \captionof{figure}{Screenshots from the agent's perspective of an episode in the grid-world and Unity environments. In both cases the instruction is \texttt{put the picture_frame on the bed}.}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.4\textwidth}
% \centering
% \begin{tabular}{cc}\hline
%   Environment & Train accuracy & Test accuracy \\ \hline
%     Grid world & 0.99 & 0.47 \\
%     Unity room & 0.99 & 0.80 \\\hline
%   \end{tabular}
%   \captionof{table}{Generalisation of an act of putting in two different environments. Both regimes involve ten red objects and a white `bed' and the same set of training and testing commands. All scores reflect the mean performance of the top three of five agent replicas (ranked by performance on the training set) per condition.}
% \end{minipage}
% \end{minipage}

% \subsection{The perspective of an agent}
% Most of our experiments have involved an agent that is `embodied' in the sense that its visual experience is highly correlated over time, and depends on its position and the direction of its field of view. This affords the agent learner a very different stream of training data than a model that learns to classify independent samples. We tested the effect of this difference on systematic generalization by devising a task that could be couched as either image-based (visual-question-answering) or as test of agent behaviour. We used the DM-Lab environment, a 3D environment that allows positions of all objects and position and viewpoint of the agent at the start of an episode to be set explicitly. As in Section~\ref{fig:blue_sunflower}, we measured the ability of the agent to generalise color-shape combinations, setting the environment so that each episode began with the agent facing two objects and the environment produced a simple color-shape instruction (\texttt{red guitar}) referring to one of the two objects. In one condition we trained an embodied agent via reinforcement learning, rewarding it for moving towards and bumping into the object matching the instruction. In a different condition, we trained a model via supervised learning to predict either \textt{Left} or \textt{Right} in response to only the first frame of the episode and the instruction. The architecture in both conditions was the same, apart from the final output layer (in one case, a fully-connected layer and softmax from the agent's memory state to a distribution over 16 motor actions and a scalar value, and in one case a fully-connected layer and softmax over two possible labels). 

% Both 



% \begin{minipage}[ht!]{\textwidth}
% \begin{minipage}[b]{0.6\textwidth}
% \centering
%     \includegraphics[width=8cm]{figures/agent_vs_image.png}
% \captionof{figure}{(a) Four (independent) training inputs from the training data for the static (visual-question-answering-style) model. (b) Four timesteps of input from a single episode for the embodied agent.}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.4\textwidth}
% \centering
% \begin{tabular}{cc}\hline
%   Regime & Train accuracy & Test accuracy \\ \hline
%     VQA & 0.99 & 0.47 \\
%     Agent perspective & 0.99 & 0.80 \\\hline
%   \end{tabular}
%   \captionof{table}{Color-shape generalisation }
% \end{minipage}
% \end{minipage}




% \subsection{The role of language}
% Prior work has demonstrated how language can serve to promote compositional behaviour in deep learning models. While the visual input to our agent in the 3D Unity room is raw and continuous, the language is synthetic and highly regular. As the agent learns, language can provide a form of supervision for how the agent should break down the world it observes, and the behaviours it can execute, into meaningful sub-parts, which in turn can stimulate generalisation.

% To verify this hypothesis, we devised a simple task in the grid world that can be solved either with or without relying on language. The agent begins each episode in a random position in the grid containing 8 randomly-positioned objects, four of one color and shape and four of another (Fig~\ref{no_lang} (a)). In each episode, one of the object types was randomly designated as `correct' and the agent received a positive +1 reward for collecting objects of this type. The episode ended if the agent collected all of the correct objects (return = +4) or if it collected a single incorrect object (reward = 0). Without access to language, the optimal policy is to simply select an object type at random and then (if possible) the remainder of that type (which returns 2 on average). In the language condition, however, the target object type (e.g. `red square') was named explicitly, so the agent could learn to achieve a return of 4 on all episodes. To test generalisation in both conditions, much like the color-shape reference expressions in Section~\ref{}, we trained the agent on episodes involving half of the possible color-shape combinations (as correct or distractor objects) and tested it on episodes involving the other half. Note that, both during training and testing, for a given correct object type there were episodes in which the incorrect objects differed in color and episodes in which the incorrect objects differed in shape\footnote{There were no episodes where the incorrect object differed in both color and shape} (so that awareness of both color and shape was necessary to succeed in general). 

% For fair comparison between the conditions, we measured performance only on test episodes in which the first object selected by the agent was correct. The progress on this metric as the agent learned the training trials is shown in Fig~\ref{fig:no_lang} (b). In line with our hypothesis, we obsrved improved generalisation in the agent with language. We note that in the more realistic (hypothetical) setting of human-machine interaction involving entirely natural language, the model would have to infer the structure in the language from less regular input (much as our agent does for vision). Inferring such structures is something networks are very good at, however [REF], so we so no reason why, in an embodied learning setting involving real language interactions, the language would not provide a similar catalyst for compositional or systematic understanding  as it does in our simulations. 


% \begin{minipage}[ht!]{\textwidth}
% \begin{minipage}[b]{0.6\textwidth}
% \centering
%     \includegraphics[width=6cm]{figures/no_lang.png}
% \captionof{figure}{A screenshot of the grid-world task that can be played with or without language. The possible goals are color-shape combinations (partitioned into train or test) that the agent either receives explicitly via a language channel or must infer from the response of the environment when it tries an object at random.}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.4\textwidth}
% \centering
% \begin{tabular}{lrr}\hline
%   Condition & Train accuracy & Test accuracy \\ \hline
%     With language & 4.0 & 3.76 & \\
%     No language & 4.0 & 3.41 & \\ \hline
%   \end{tabular}
%   \captionof{table}{TODO: update this and update the numbers to be accuracies}
% \end{minipage}
% \end{minipage}



% \andrew{In some ways I feel like it would be useful to briefly mention the blue sunflower experiments here too, as they seem to provide a slightly different notion of what encourages systematicity -- in particular variation you've seen along the same axis in different contexts can encourage more ``concept-like'' understanding with something you only see once. I see this as being related to more general transfer effects, like the fact that e.g. pretraining on imagenet is useful for classifying satellite images (https://core.ac.uk/download/pdf/31020721.pdf) which is a quite different data distribution. Seeing large amounts of variability can help the model to pick out the ``object-like'' things that are important in a related domain.}

\subsection{Abstracting across the training set}

In all of our experiments, our agents are trained with a degree of procedural variation in the tasks that they attempt and certain environmental factors. To show how this variation can drive systematicity even in highly controlled domains, we designed a simple grid-world experiment that tested our agent's ability to combine shape and color words in a systematic way (This ability of multi-modal agents to generlize shape-color composition has already been established in several prior studies [REF]). In our grid world, the agent receives a RGB pixel representation of the world from a top-down perspective, including a square indicating its current position. The agent can take one of four actions (\texttt{UP, DOWN, LEFT, RIGHT}) to move around the world. At the start of each episode, the agent receives a two-symbol instruction (\texttt{red triangle}) indicating the colour and the shape of the target object. If the agent moves into the target object before the episode ends, it receives a positive reward, and if it moves into the (incorrect) distractor object or the time runs out it receives no reward. Each episode ends after 30 timesteps or when the agent moves into the square occupied by one of the objects. Over the course of multiple episodes, the agent learns how these symbols correspond to its visual observations and develop a language-conditional policy of moving towards the correct object when instructed. 

To evaluate generalisation, the available colors and shapes in the environment were partitioned into sets $S = \mathbf{s} \cup \hat{\mathbf{s}}$ and $C = \mathbf{c} \cup \hat{\mathbf{c}}$. We then train the agent on episodes with instructions sampled from one of the sets $ \mathbf{c} \times \mathbf{s}$, $\hat{\mathbf{c}} \times \mathbf{s}$ or $ \mathbf{c} \times \hat{\mathbf{s}}$, and, once trained, we evaluate its performance on instructions from $ \hat{\mathbf{c}} \times \hat{\mathbf{s}}$. Importantly, to ensure all parts of the referring expression in the instruction are necessary, during both training and testing the agent faces trials in which the distractor object either matches the color of the target object or the shape of the target object. Figure X shows that the agent exhibits good ability to generalise (recombining shape and color terms into novel combinations) even when the sets $\mathbf{s}, \mathbf{c}, \hat{\mathbf{s}}, \hat{\mathbf{c}}$ contain a small number of factors from which to learn. 

\begin{table}
	\begin{minipage}{0.25\linewidth}
		\centering
		\includegraphics[width=40mm]{figures/color_shape.png}
		%\captionof{figure}{2-D scatterplot of the Student Database}
		\label{test}
	\end{minipage}\hspace*{\fill}
	\begin{minipage}{0.2\linewidth}
		\label{table:student}
		\centering
		\begin{tabular}{llllrr}
			\toprule
			C  & S & $\hat{C}$ & $\hat{S}$ & Tr & Te \\
			&&&&&\\ \midrule
			&&&&&\\ \bottomrule
		\end{tabular}
	\end{minipage}\hspace*{\fill}
	\begin{minipage}{0.25\linewidth}
		\centering
		\includegraphics[width=40mm]{figures/color_shape_sunflower.png}
		%\captionof{figure}{2-D scatterplot of the Student Database}
		\label{test}
	\end{minipage}\hspace*{\fill}
	\begin{minipage}{0.2\linewidth}
		%\caption{Student Database}
		\label{table:student}
		\centering
		\begin{tabular}{llrr}
			\toprule
			C  & S & Tr & Te \\
			\midrule
			 2 & 2  & 1.00 & 0.64  \\
			 9  & 2  & 1.00 & 0.80 \\
			\bottomrule
		\end{tabular}
	\end{minipage}
\caption{Zero-shot generalisation of (color-shape) object referring expressions for different training regimes. Left almost perfect systematic generalisation is observed when all shapes are observed during training with some variety of different colors. Right, generalisation is above 80\% accuracy (chance = 0.5) for shapes observed with a single colour during training; this capacity grows with the number of colors ($\vert \mathbf{c} \vert$) that \emph{other} shapes in the training set are observed with. All scores reflect the mean performance of the top three of five agent replicas (ranked by performance on the training set) per condition.}
\end{table}

The assumption that all objects and shape-words can be encountered in a range of different colours is not particularly realistic. In the experience of a human learner, certain objects might be experienced in multiple colours (such as toys) while others (such as fruits) will have a single colour, but we can understand expressions like \emph{purple banana} without direct experience of such a thing. To test this capacity, we trained the agent on instructions sampled either from a set $ \mathbf{c} \times \mathbf{s}$ or from a set $ \{c\} \times \hat{\mathbf{s}}$ where $c$ is a single color. We then evaluated the trained agent on episodes with target object descriptions from $\mathbf{c}\times \hat{\mathbf{s}}$. The shapes in the set $\hat{\mathbf{s}}$ play the role of banana in the example above, while $c$ is its typical color yellow. As shown in Fig~\ref{fig:blue-sunflower}, we find that the agent can understand the `banana` terms $\hat{\mathbf{s}}$ described in conjunction with colors other than yellow in 80\% of episodes. Interestingly, this capacity increases as the variety of colors that \emph{other} shapes in the training set are observed with increases. This suggests that the experience of shapes that vary widely in color (the fully green area of the training regime in Fig~\ref{fig:blue-sunflower}) are critical to the development of color as a separable and recombinable aspect of experience, the knowledge of how color words refer to this, and the ability to apply this knowledge, in theory, to any shape whatsoever. 

The `blue sunflower` analysis shows that agents operating in a grid-world can learn to generalize systematically given sufficient variation in theiry training data. However, in the cases the more realistic environment 3D Unity room, we observed systematic generalisation with making a particular effort to involve many factors of variation in the training data. This suggests that environmental realism in general (rather than explicit variation in directly-relevant factors or words) might play an important role in stimulating emergent systematicity.

To test this hypothesis explicitly, we compared the generalisation of an agent trained to lift objects and to put them on a bed (as in Section~\ref{sec:put_lift_generalisation}), when trained in both a  (more realistic) Unity room and a (more abstract) grid world. At a certain level of abstraction, the tasks in the two environments were identical; each episode involved three red objects and a white object positioned at random in a room. In `lifting' trials, the agent in both cases had to visit a specific red object, and in `putting' trials, the agent had to pick up a specific object and move with that object to the bed. There was a total of seven possible red objects in both cases, of which all were involved with `lifting' trials during training but only three in `putting' trials. The test trials consisted of `putting' trials with the remaining four objects. While the task are identical at a conceptual (and linguistic) level, the experience of an agent doing the task in the the grid world was quite different from that in the Unity room. In the grid world, the agent observed the whole world (including itself) from above, and could move to only 49 possible locations by taking one of four possible actions. 

As shown in figure X, agents in both conditions were able to master the training set with almost perfect performance. However, on the test set, the performance of the agent in the Unity room was far better than the agent in the grid world. Failure cases of agent in the grid world can be observed in the video REF; it typically exhibits less certainty, putting the wrong object on the bed or running out of time before it is able to make a decision. 

Many studies that have observed limited systematic generalisation in neural network-based models involve synthetic symbolic data [REF] or abstract grid environments [REF]. This led to a hypothesis that emergent systematicity might in fact be supported by environmental richness. 










\section{Introduction}
Since the earliest days of research on neural networks, a recurring point of debate is whether neural networks exhibit `systematic' generalization~\citep{fodor1988connectionism,marcus1998rethinking,mcclelland1987parallel}. This debate has been re-energized over the past few years, given a resurgence in neural network research overall \citep{lake2017generalization, bahdanau2018systematic, lake2019compositional}. The current evidence reveals that systematicity in neural networks is \emph{not} a binary question; since there are cases where networks behave systematically and others where they do not, a more pertinent research question is \emph{when} and under \emph{what conditions} neural networks are systematic. 
% Systematicity is a desirable property for many potential AI applications, so it is therefore critical to better understand \emph{when} or \emph{under what conditions} we can expect neural networks to generalize in systematic ways.
Here, we establish that a conventional neural-network-based agent exposed to raw visual input and symbolic (language-like) instructions readily learns to exhibit strong systematic generalisation, and explore the conditions that support the emergence of this behaviour. First, we show in a 3D simulated room that an agent trained to \instr{find} all objects from a set and \instr{lift} only some of them can \instr{lift} withheld test objects never lifted during training. Second, we show that the same agent trained to \instr{lift} all of the objects and \instr{put} only some of them during training can \instr{put} withheld test objects, zero-shot, in the correct location. 
%Third, we show how this propensity to extend predicates to novel arguments applies not only to concrete motor actions and verbs, but to abstract modifiers like negation. When trained on positively posed finding commands (\instr{find a teddy bear}) for all the objects, and negatively posed commands (\instr{find [something that is] not a toy train}) for only some of them, the agent can again interpret, with above chance accuracy, negatively-posed commands involving withheld test set objects (\instr{find not a teddy bear}). 
Because the architecture of our agent does not include components that are explicitly engineered to promote systematicity, we refer to the behaviour it exhibits as \emph{emergent systematicity} \citep{mcclelland2010letting}.

In order to better understand emergent systematicity, we conduct several  experiments to isolate its contributing factors. We find three to be critical: (a) the number of words and objects experienced during training; (b) a bounded frame of reference or perspective; and (c) the diversity of perceptual input afforded by the temporal aspect of the agent's perspective. %Factor (a) is demonstrated in the context of a negation generalisation experiment, in which the agent is able to generalise, above chance accuracy, to unseen negatively-posed commands (\instr{find } [something that is] \instr{ not a toy train}) if it is provided with enough training examples.
%trained on positively posed finding commands (\instr{find a teddy bear}) for all the objects, and negatively posed commands (\instr{find [something that is] not a toy train}) for only some of them. We find that, if the agent is provided with enough training examples, it can again interpret, with above chance accuracy, negatively-posed commands involving withheld test set objects (\instr{find not a teddy bear}). 
These results serve to explain differences between our findings and studies showing poor systematicity, where networks were typically trained in a supervised fashion on abstract or idealised stimuli from a single modality \citep{lake2017generalization}. They also suggest that the human capacity to exploit the compositionality of the world, when learning to generalize in systematic ways, might be  replicated in artificial neural networks if those networks are afforded access to a rich, interactive, multimodal stream of stimuli that better matches the experience of an embodied human learner \citep{clerkin2017real,kellman2000cradle,james2014young,yurovsky2013statistical,anderson2003embodied}.



\subsection{Systematicity and neural networks}

Systematicity is the property of human cognition whereby ``the ability to entertain a given thought implies the ability to entertain thoughts with semantically related contents" \citep{fodor1988connectionism}. As an example of systematic thinking,  \cite{fodor1988connectionism} point out that any human who can understand \emph{John loves Mary} will also  understand the phrase \emph{Mary loves John}, whether or not they have  heard the latter phrase before. Systematic generalization~\citep{plaut1999systematicity,bahdanau2018systematic,lake2019human} is a desirable characteristic for a computational model because it suggests that if the model can understand components (or words) in certain combinations, it should  also understand the same components in different combinations. Given that human reasoning is often not perfectly systematic~\citep{o2013limited}, here, we consider systematicity to be a question of degree, rather than an absolute characteristic of an intelligent system. Note that systematic generalisation is also sometimes referred to as `combinatorial generalization'~\citep{o2001generalization,battaglia2018relational}. 

Recent discussions around systematicity and neural networks have focused on the issue of how best to encourage this behaviour in trained models. Many recent contributions argue that systematic generalziation requires inductive biases that are specifically designed to support some form of symbolic computation (such as graphs~\citep{battaglia2018relational}, modular-components defined by symbolic parses~\citep{andreas2016neural,bahdanau2018systematic}, explicit latent variables~\citep{higgins2017scan} or other neuro-symbolic hybrid methods~\citep{mao2019neuro}). On the other hand, some recent work has reported instances of systematicity in the absence of such specific inductive biases \citep{chaplot2018gated,yu2018interactive,lake2019compositional}. In the following sections, we first add to this latter literature by reporting several novel cases of emergent systematicity. Unlike in previous work, the examples that we present here involve tasks involving the manipulation of objects via motor-policies, as well as language and vision. This is followed by an in-depth empirical analysis of the environmental conditions that stimulate systematicity in these cases.
